Data Appraisal Without Data Sharing

One of the most effective approaches to improving the performance of a machine learning model is to procure additional training data. A model owner seeking relevant training data from a data owner needs to appraise the data before acquiring it. However, without a formal agreement, the data owner does not want to share data. The resulting Catch-22 prevents efficient data markets from forming. This paper proposes adding a data appraisal stage that requires no data sharing between data owners and model owners. Specifically, we use multi-party computation to implement an appraisal function computed on private data. The appraised value serves as a guide to facilitate data selection and transaction. We propose an efficient data appraisal method based on forward influence functions that approximates data value through its first-order loss reduction on the current model. The method requires no additional hyper-parameters or re-training. We show that in private, forward influence functions provide an appealing trade-off between high quality appraisal and required computation, in spite of label noise, class imbalance, and missing data. Our work seeks to inspire an open market that incentivizes efficient, equitable exchange of domain-specific training data.

==> mpc.tex <==
\section{Secure Multiparty Computation (Extended)}
\label{app:mpc}
Despite MPC's suitability for private machine learning, MPC requires special software to be performant, which can be engineering-intensive. Notably, floating point arithmetic, comparisons, and nonlinearities are approximated on a case-by-case basis to balance accuracy, runtime, communication, memory, and numerical stability. Consequently, machine learning researchers need to adopt interfaces in addition to their training in order to take advantage of secure MPC. Recently, emerging private machine learning frameworks afford expressive machine learning activities in private ~\citep{sealcrypto, ludwig2020ibm, crypten}. In particular, CrypTen~\citep{crypten} allows PyTorch-like implementation of machine learning models in private. In doing so, it supports private auto-differentiation of a plaintext model after applying encryption. The appraisal methods in Section~\ref{sec:private_appraisal} are thus implemented according to their PyTorch equivalents. We note that all CrypTen experiments in this work require no additional change except for precision adjustment, which is set to 16 bits (default 12).

An additional complication pertains to the workflow of machine learning development. Without an appraisal and transaction phase, private training often presumes that the data is exclusively applied to a particular model and never revealed. Such rigid MPC setup for model training can be unappealing. In the clear, a researcher often owns both data and models, yet still require external data. If that data is never revealed, the researcher loses the ability to monitor key metrics, debug data, and potentially the ability to tweak their model architecture, all of which are typical to the workflow of model developers. Our work, in contrast, aids model owners with appraisal values computed in private, prior to the exchange of data. Thus data transaction may be in the clear to maximize flexibility.

==> prior.tex <==
\section{Related Work}
\label{sec:prior}
\paragraph{Private Data Appraisal.}
Private data appraisal is studied with differential
privacy~\citep{li2014theory} and federated learning~\citep{song2019profit,
wang2019measure, wang2020principled}.
However, the problem setting considered in these
studies is different from the setting studied in our work. Their setup is designed for assessing sets of data \emph{after} the model is trained on them. The exchange of data in these
applications is treated as foregone conclusion, with the private pricing serving
as a mechanism to incentivize more data contributions. In contrast, our setup dictates that the assessment necessarily predates the decisions to include the training data. This lets the model and data owners decide if it is worth
engaging in the transaction based on the appraised value.
Finally, our proposed influence-based appraisals are computed without incurring the computational intensity of training. While their methods often involve repeated training in private, the computational intensity of private influence computation is approximately that of only one pass of private gradient updates.

\paragraph{Data Market Dynamics}
A primary motivation for our work is to enable efficient data markets for low-resource projects.
Many have surmised the rise of a data market for the sole purpose of trading training data for machine learning models. We expand on that promise by realizing an efficient privacy-perserving appraisal by applying multi-party computation, solving primarily the incentives problems in a noisy market. However, our focus on crafting the appraisal
to suit privacy constraints only fills in a small part of the whole puzzle;
\citet{azcoitia2020try} proposes Try Before You Buy, by supposing heuritstic evaluations that
can be of linear runtime with respect to the number of data owners. They further prove the efficiency of various acquisition strategies, while we presume in our work.

\paragraph{Shapley Values.}
Over concurrent datasets, Shapley values from ~\citet{shapley1952value} have been proposed as an equitable method for data appraisal~\citep{ghorbani2019data,
jia2019towards, azcoitia2020try, azcoitia2020computing}. A primary motivation of Shapley values over influence-based
approaches is the invariance to the order of data aquisition. Instead, we focus on the case where the order of acquisition is important, as earlier acquisition decisions may justifiably affect the perceived value of data that arrive later. We thus pursue valuation techniques based on leave-one-out training.
% A one-by-one evaluation has some additional benefits. Suppose a data owner fears similar or duplicate data to be available, which will render their data less useful if included prior to evaluation, the data owner may be eager to participate at soon as the submission window begins. This incentive may be especially useful for low resource settings.

\paragraph{Influence Functions.}
Assessing the impact of data to a statistical model is by itself a long studied subject. A natural method defines the impact through leave-one-out training. Measuring the effect of the data under leave-one-out training is known as Cook's
distance in linear regression~\citep{cook1977detection} or the influence curve in regression residuals~\citep{cook1982}.
Many contemporary works employ influence functions to explain existing training examples aposteri, including for interpretability~\citep{koh2017, guo2020fastif}, efficient cross-validation~\citep{giordano2019swiss}, and efficient training data
removal~\citep{guo2019certified, koh2019accuracy}. As a result, influence functions are usually 1. defined with respect to the trained model, 2. used to approximate parameter change under data removal.
For non-convex models,~\citet{basu2020influence} finds the approximation errors for those influence functions sensitive to depth, regularization, and data composition, part of which~\citet{basu2020second} mitigates by expanding influence to include second order terms in the approximation.

However, little attention is paid to appraising datasets prior to training. Evaluating the expected utility of training examples is instrumental to efficient data exchanges, where existing model and additional data belong to separate individuals. Most recently,~\citet{raj2020model} applies forward influence functions to quickly select unseen training samples for model selection. They find that for sufficient training data, the first order approximation of the model's test loss through (forward) influence functions is valid, under convexity, smoothness, good regularization, and bounded gradients. Like our setup,~\citet{raj2020model} seeks to evaluate between candidate examples prior to training, approximating the data's relative importance rather than predicting the exact parameter change or losses. Our work expands the method to perform data evaluation and selection in private, achieving computational gains against retraining in secure MPC. Finally, we are primarily concerned with enabling data transaction rather than active learning. While experiments in~\citet{raj2020model} select a pool of samples from uncorrupted training data, our setup adds substaintial noise to the candidate data sets to simulate an open data market.

\paragraph{Challenges to Influence-Based Approximations}
In deep learning, influence functions are found to be sensitive to hyperparameters, such as architecture and regularization strength, and particularly reliant on convex loss and shallow networks~\citep{basu2020influence}.
Additionally, for groups of data, the makeup of the group and its size affect the approximation error~\citep{koh2019accuracy, basu2020second}.

Nevertheless,~\citet{basu2020second, basu2020influence} acknowledge that after summing up a set of influences, as we do in Equation~\ref{eq:influence}, peculiarities in individual samples' influence approximations matter less.
% the appraisal function outputs a scalar value (smoothed signal)
Furthermore, in our data market setup, it is only desired that influence functions retain the value ranking among potential datasets under the realistic constraints, such as noise, class imbalance, and missing data. As the candidate dataset size and model architecture are assumed constant, as both belong to the model owner, group size and inter-architecture differences that make influence functions fickle become irrelavant. Finally, the datasets to evaluate under forward influence are often not part of the training set. This novel use case lets influence functions differentiate between data sets that may diverge greatly from the initial training and testing sets, for which they are empirically informative.

\paragraph{Coreset Selection.}
For actively selecting unseen data, a closely related problem looks at using gradient information for subset selection by deriving a scaler when evaluating the empirical risk minimization with every data set is impractical \citep{munteanu2018coresets, raj2020model}. Influence functions, especially the additive variety akin to~\citet{koh2017, giordano2019swiss}'s first order formulation, can be used as an alternative to ranking datasets without the computation. In particular,~\citet{raj2020model} suggests greedy additions of top-ranking training samples using influence functions to fast iterate over model selection process. However, a coreset selection framework is more approproiate for choosing multiple sets of data. Instead, we focus on selecting just one dataset at a time, which ignores the interactions between different candidate datasets.

==> related.tex <==
\section{Related Work (Extended)}
\label{app:related}
%Shapley values~\cite{shapley1952value} have been proposed as an equitable method for data appraisal~\cite{ghorbani2019data,
%jia2019towards}. However, a primary motivation of Shapley values over influence-based approaches is the invariance to the order of data aquisition. Instead, we focus on the case where the order of acquisition is important, as earlier acquisition decisions may affect our judgement for the value of data that is available later. Instead we opt for using leave-one-out influence-based valuation techniques.

%Prior work also considers private data appraisal with differential privacy~\cite{li2014theory} and federated learning~\cite{song2019profit,
%wang2019measure, wang2020principled}. The setup is designed for assessing sets of data after the model has trained on them; in contrast, our setup dictates that the assessment necessarily predates the decisions to include the training data. Our proposed influence method also computes the appraisal without incurring the computational intensity of training.

%Assessing the impact of data to a statistical model is by itself a long studied subject. A natural method defines the impact through leave-one-out training \cite{cook1977detection, cook1982}. Influence functions have been proposed as an efficient way to evaluate training data aposteri \cite{koh2017, giordano2019swiss, guo2019certified, koh2019accuracy, guo2020fastif}. Yet, for non-convex models, ~\cite{basu2020influence} finds the approximation errors for influence functions, defined on a model post training, to vary highly based on depth and regularization and data composition, part of which can be mitigated by expanding the influence functions to include second order terms in the approximation ~\cite{basu2020second}.

%Meanwhile, evaluating data \emph{before} training is not widely explored. By modifying influence functions for unseen data, ~\cite{raj2020model} applies forward influence functions to select the top datasets, thus speeding up model selection. In contrast, we apply it to tackle private data transaction. Additionally, we simulate real world data markets where the initial empirical distribution may be insufficient and widely different from the desired target, and the data sets submitted for evaluation may be noisy and imbalanced.

\subsection{Influence Functions}
Measuring the effect of the data under leave-one-out training is known as Cook's
distance in linear regression~\cite{cook1977detection} or the influence curve in regression residuals~\cite{cook1982}. Many contemporary works employ influence functions of explaining existing training examples a posteri, including for interpretability~\citep{koh2017}, efficient cross-validation~\cite{giordano2019swiss}, and efficient training data
removal~\cite{guo2019certified, koh2019accuracy}. As a result, influence functions are defined with respect to the trained model.

However, little attention is paid to appraising datasets prior to training. Evaluating the expected utility of training examples is instrumental to efficient data exchanges, where existing model and additional data belong to separate individuals. Most recently, ~\cite{raj2020model} uses forward influence functions to rank datasets for faster model iteration. They find that for sufficient training data, the first order approximation of the model's test loss through (forward) influence functions is valid, under convexity, smoothness, good regularization, and bounded gradients. Like our setup, ~\cite{raj2020model} seeks to evaluate between candidate examples prior to training, approximating the data's relative importance rather than predicting the exact losses. Our work expands the method to perform data eveluation and selection in private, utilizing the gains in computation against retraining in secure multi-party computation.

\subsubsection{Criticism of Influence Functions}
In deep learning, influence functions are found to be sensitive to hyperparameters, such as architecture and regularization strength, and particularly reliant on convex loss and shallow networks ~\cite{basu2020influence}.
Additionally, for groups of data, the makeup of the group and its size affect the approximation error~\cite{koh2019accuracy, basu2020second}.
However, ~\cite{basu2020second, basu2020influence} acknowledges that after summing up a set of influences, peculiarities in individual approximations matter less.
Furthermore, in our data market setup, it is only desired that influence functions retain the value ranking among potential datasets under the realistic constraints, such as noise, class imbalance, and missing data.
As the candidate dataset size and model architecture are assumed to be constant, group size and inter-architecture differences become irrelavant.
Finally, the datasets to evaluate are often not part of the training set.
This novel use case lets influence functions differentiate between data sets that may diverge greatly from the initial training and testing sets, for which they are empirically informative.


\subsection{Shapley Values}
Because the value of data may affect the decision to transact or exclude, appraisals need to be done in private. Over concurrent datasets, Shapley values~\cite{shapley1952value} have been proposed as an equitable method for data appraisal~\cite{ghorbani2019data,
jia2019towards}. A primary motivation of Shapley values over influence-based
approaches is the invariance to the order of data aquisition. Instead, we focus
on the case where the order of acquisition is important. As earlier acquisition decisions may affect our judgement for the value of data that is available later, we opt for using
leave-one-out and influence-based valuation techniques instead.

\subsection{Coreset Selection}
For actively selecting unseen data, a closely related problem looks at using gradient information for subset selection by deriving a scaler when evaluating the empirical risk minimization with every data set is impractical \cite{munteanu2018coresets, raj2020model}. Influence functions, especially the additive variety akin to ~citep{koh2017, giordano2019swiss}'s first order formulation, can be used as an alternative to ranking datasets without the computation. In particular, ~\cite{raj2020model} suggests greedy additions of best data sets using influence functions to fast iterate over model selection process.

\subsection{Private Data Appraisal}
Private data appraisal is studied with differential
privacy~\cite{li2014theory} and federated learning~\cite{song2019profit,
wang2019measure, wang2020principled}.
However, the problem setting considered in these
studies is different from the setting studied in our work. The exchange of data in these
applications is treated as foregone conclusion, with the private pricing serving
as a mechanism to incentivize more data contributions.
In contrast, our protocol allows the appraisal to be performed in private prior to the transaction.
This lets the model and data owners decide if it is worth
engaging in the transaction based on the appraised value.
Finally, while their methods often involve repeated training in private, the computational intensity of private influence computation is akin to that of one pass of private gradient updates.



